Creating a Domain-diverse Corpus for Theory-based Argument Quality Assessment

Computational models of argument quality (AQ) have focused primarily on assessing the overall quality or just one specific characteristic of an argument, such as its convincingness or its clarity. However, previous work has claimed that assessment based on theoretical dimensions of argumentation could benefit writers, but developing such models has been limited by the lack of annotated data. In this work, we describe GAQCorpus, the first large, domain-diverse annotated corpus of theory-based AQ. We discuss how we designed the annotation task to reliably collect a large number of judgments with crowdsourcing, formulating theory-based guidelines that helped make subjective judgments of AQ more objective. We demonstrate how to identify arguments and adapt the annotation task for three diverse domains. Our work will inform research on theory-based argumentation annotation and enable the creation of more diverse corpora to support computational AQ assessment.

==> 3.1-annotation-setup.tex <==
\jttodo{one big thing with the paper is there is no real comparison to Wachsmuth 2017a who also simplified (right?). We should make it clear the differences between our approach and theirs. CN: they didn't do any simplifying}
\joeltodo{responding to CN above.  So does that undercut the significance of what we have done if they were able to crowdsource this without simplification?  } \altodo{They explicitely say in their paper as a conclusion that the task should be simplified and we show that our agreement on the same data is better than theirs, so I think it is fine.}
% \jttodo{another major issue is WHY we are simplifying.  it's not like we made a simpler process which gets the same information as the original scheme.  We actually simplify the actual scheme.  So it kind of makes sense that scores would increase.}
% We describe the preliminaries of our annotation study.

% \paragraph{Theory-based Argument Quality.}


\newcite{wachsmuth-etal-2017-computational} developed a taxonomy of AQ synthesized from traditional works in argumentation theory, such as \newcite{kennedy2007aristotle}.
The full taxonomy is depicted in Figure \ref{fig:tax}, and defines the Overall AQ to consist of the following three subdimensions, each of which is itself defined by several finer-grained AQ aspects:

\begin{wrapfigure}{r}{0.48\textwidth}
  %\begin{center}
    % \vspace{-8mm}
    \includegraphics[width=\linewidth,trim=0.3cm 0cm 0.3cm 0cm]{img/taxonomy.pdf}
  %\end{center}
  \caption{The taxonomy of theory-based argument quality aspects~\cite{wachsmuth-etal-2017-computational}.}
  \label{fig:tax}
\end{wrapfigure}

% \jttodo{it seems redundant to list the domains in a general sense below but then go into detail in Sec 3.3}
\vspace{0.5em}
 \noindent\emph{Cogency} relates to the logical aspects of AQ, for instance, whether the an argument's premises are acceptable (local acceptability) or whether they can be seen as relevant for the conclusion (local relevance).
 
 \vspace{0.5em}
 \noindent\emph{Effectiveness} indicates the rhetorical aspects of an argument. Aspects of effectiveness include, for instance, its clarity, or its emotional appeal.
 
 \vspace{0.5em}
 \noindent\emph{Reasonableness} reflects the quality of an argument in the overall context of the discussion, as, for instance, its relevance towards arriving at a resolution of the issue (global relevance).


% %% MOVED TO 3.3 
% \paragraph{Domains.} In total, our study covers three domains: (1) Debate forums (Debates), (2) Q\&A forums (Q\&A), and (3) Review forums (Reviews).
%  While Debates are generally well-explored in computational AQ \cite{habernal-gurevych-2016-argument}, only a few works exist on Q\&A and Reviews.
 
%  \vspace{0.5em}
%  \noindent\emph{Debates.} Online forums, in which, typically, given a topic or motion, users can define their stance (\emph{pro}/\emph{contra}) and write and argument which supports their stance.
 
%  \vspace{0.5em}
%  \noindent\emph{Q\&A.} Online forums, in which users can seek for help or ask any question, which they'd like to be answered by other users. In contrast to debates, Q\&A allow for more freedom and argumentative and non-argumentative posts are relatively mixed.
 
%  \vspace{0.5em}
%  \noindent\emph{Reviews.} Online forums, which allow users to rate a product or a business. Typically, the overall satisfaction is depicted by some kind of star rating, in addition to which users provide a free text answer.
 
%  \vspace{0.5em}
%  \noindent Later, we describe how we collected data representing each of the domains and how we adapted our annotation guidelines.
 

% \cntodo{this needs to be moved}\paragraph{Contributors.} 
% Throughout our study, we distinguish between two groups of annotators: (1) expert annotators and (2) crowd annotators.

% Each expert annotator is a fluent or native English speaker with an advanced degree in linguistics.
% Experts underwent training, which included studying guidelines and participation in calibration tasks.
% The authors facilitated meetings with experts during pilot annotation to improve the guidelines and to calibrate judgements.
% Experts all participated in pilot tasks for annotation of new domains and provided feedback on domain-specific guidelines before each domain was launched to the crowd.

% \todo[color=green]{Do we want to discuss open crowd vs. channel partner crowd? cn: no}
% All crowd contributors are native or fluent English speakers engaged through Appen (formerly Figure Eight).
% Crowd contributors did not participate in calibration meetings or receive any direct feedback from the authors.
% All feedback was relayed to contributors through a liaison.\\
% - 10 judgments per instance\\ 
% - paid \$.45-\$.65 per judgment (increased over time) to ensure \$21 per hour. 
% manually reviewed each crowd workers judgments to block those underperforming and used MACE and Krippendorff to assess annotators\\
% selecting crowd workers: OC vs. CP, manual review, agreement, MACE\\
% - We could also report the comparison LC vs. CP vs. OC on pilot 8 and 9\\
% - Especially when computing the mean, our crowd workers votes are close to the expert annotations, and at times clearly higher than the ones reported in the original paper (see the final row entitled \textsc{TvsP}).\\

==> analysis.tex <==
\section{Analysis}
\begin{figure}
    \centering
    % \includegraphics{}
    \missingfigure
    \caption{table of alpha results}
    \label{fig:my_label}
\end{figure}
We calculate Krippendorff's alpha to analyze inter-annotator reliability within the pool of expert annotators, crowd annotators, and across these cohorts.\\
- agreement within group per domain\\
- agreement b/w groups per domain\\
- \todo[color=green]{should Wachsmuth be here or in the pilots section?}compare to Wachsmuth results (most-agreeing pair?)\\
--- FROM MODEL PAPER: The Dagstuhl-ArgQuality-Corpus\footnote{\url{http://argumentation.bplaced.net/arguana/data}} (\textsc{DS})~\cite{wachsmuth-etal-2017-computational} was presented in combination with the taxonomy of argument quality described above and consists of $320$ web debate arguments annotated with all $15$ argument quality aspects. 
The arguments were originally taken from UKPConvArgRank~\cite{habernal-gurevych-2016-argument}. 
We use the corpus in pilot studies in order to estimate the quality of our annotations.\cntodo{by comparing with the wachsmuth ratings}\\
\begin{figure}
    \centering
    % \includegraphics{}
    \missingfigure
    \caption{annotated examples for qualitative analysis}
    \label{fig:my_label}
\end{figure}
- add tables or plots that show the scores across different domains and dimensions\\
- qualitative analysis of dimensions across domains (why dimension score is low in particular domain)\\
- correlations b/w dimensions across domains\\
(i) IAA: The average of valid annotators reliability scores on the quality annotations is 0.12. 
This task reproduces the task from Toledo et al. (2019), and as established there, such an
average is acceptable due to the subjectivity of the task.
Among other things, Toledo et al. (2019) rely on the taskaverage-κ of the stance annotations in the same task, which was 0.69 in that work, and here it is 0.83.\\

(k) agreement/disagreement: 
\todo{this shouldn't be its own section. should work results into narrative.}
someone will ask how we resolved disagreements and how often during the annotation process.\\
examples: Figure \ref{fig:ex2} shows a second difficult example from the pilot studies, which argues against abortion.
Their argument, however, starts with a quoted passage in favor of abortion, which is then defeated throughout the rest of the argument. 
Without further context, one is unable to establish whether this passage is an actual citation or not -- no reference is provided.\footnote{Note that there is also no context available in the IAC corpus.} 
While this was seen as an example of the \textit{straw man fallacy}~\cite{Walton1996-WALTSM-4} by annotator~$2$, which might be \textit{effective} for an online forum but not \textit{reasonable} at all, annotators~$1$ and $3$ found a) it confusing how the counterargument was presented and b) the offensive language negatively dominating the effectiveness dimension.
Furthermore, they gave a higher score on \textit{Reasonableness} than annotator~$2$ as they thought a counterargument was anticipated.
At the same time, however, the intra-group agreement is low,\jttodo{we'll need to watch that this (low intra agreement) doesn't become a red herring} highlighting the difficulty and high subjectivity of the task.\cntodo{what about the expert intro-group agreement?}
The final agreement reached on our corpus is depicted in Table ....\altodo{Compute and add final agreements? LN: this doc has all agreement info: $https://docs.google.com/document/d/12EHT3IU1JmTPVgr21u6fAZ5IHfEKoGxh_9ZqWsPILuE/edit$ -- this doc has not the final agreements}\\
\\

\\

...do mean scores conflate to the middle\\
\\
methods for combining the judgments and different statistics to measure IAA, etc.\\
\\
Other things to add here if we'd like that: Correlation analysis, histogram?, good+bad quality example..




==> corpus-numbers.tex <==
DEBATE\\
We presented 600 instances from CM and CMV to 3 expert annotators.
Of these instances, 551 are judged as argumentative based on a 0.6 majority.
We then present each expert with 200 instances to be singly-annotated.
Across these batches, a total of 548 instances are found to be argumentative.
This results in a total of 1,099 expert-annotated argumentative instances.\\
Crowd workers judged 900 different instances, of which 781 were judged argumentative based on a 0.5 majority.
The crowd then scored 538 instances judged as argumentative by the majority of experts.
\\
YAHOO\\
In our annotation study, we only include answers that a majority of raters (6/10) labeled \textit{argumentative} (this threshold was selected by manual inspection).  \jttodo{do we have statistics on how well Turkers fared at this task?  Someone is going to ask this...}\altodo{I have Krippendorff for all MTurk tasks -LN}\\
625 instances presented to 3 experts, 546 arg with majority = 2/3\\
626 for single annotation with 2 experts, 498 argumentative across batches.\\
total 1,044 argumentative instances from experts\\
crowd judged 834 instances, 809 argumenatative\\
judged 500 argumenatative instances from experts with maj = 2/3
\\
YELP
600 double-annotated by experts, all 600 argumentative\\
crowd scored 500 intances, 497 argumentative\\
crowd scored 100 argumentative instances from experts\\


==> pilot-info.tex <==
\todo{work the different pilots into the narrative instead of having one section on pilots. exclude the ones that do not fit into the narrative. "a series of pilots" with a focus on the most impactful pilots. can this pilot help other researchers design a task?}
Before corpus creation, we ran a series of pilots to prepare for large-scale annotation of domains not previously annotated for argument quality.
The purpose of the pilots was to refine the guidelines and simplify the task.
We experimented with the annotation schema, data sources, and scale used for scoring. 
We collected feedback from experts and measured inter-annotator agreement using Krippendorff's alpha to analyze pilot results.
\begin{comment}
Goals of the pilots
1. scale: 3 or 5
2. annotators (crowd v. channel v. experts)
3. reduced dimensions
4. data 

Brainstorming:
- Just include a pilot dataset (consisting of all potential datasets)
- crowdsource annotators = channel partner (don't mention open crowd)
\end{comment}
\todo[color=green]{add number instances for each pilot}
\paragraph{Round 1 (pilots 1-3)}
- GOAL: feasibility of new domains, testing sources within domains (e.g., ConvinceMe vs. 4Forums) \todo [color=green]{is this correct?}, iterating on guidelines\\
- PARTICIPANTS: authors + experts in linguistics w/ advanced degrees\\
- SETUP: all dimensions, all data, 3pt scale\\
- ROUND 1 AGREEMENT\\
- RESULTS: decided on data to use for large-scale annotation
\paragraph{Round 2: (pilots 4-6)}
- GOAL: reduced dimensions + 5pt scale (Dagstuhl)\\
- SETUP: data used:\todo[color=green]{confirm with Anne} ?,\\  Pilot 4: all dimensions, 3-point scale\\
Pilot 5a: reduced dimensions, 3-point scale\\
Pilot 5b: reduced dimensions, 5-point scale\\
Pilot 6a: same as 5a\\
Pilot 6b: same as 5b\\
\todo[color=green]{consider including only one of pilot 5 or 6 since they were same}
- ROUND 2 AGREEMENT\\
- RESULTS: reduced dimensions with a 5-point scale\\
- The feedback we collected from our linguistic expert annotators confirmed the suitability of this decision.\cntodo{also made the task easier for the experts} TODO: Maybe talk about binary score?\\
\paragraph{Round 3 (pilots 7-12)}
- GOAL: feasibility of crowd v. experts\\
- SETUP: Pilot 7: reduced dimensions, 5-point scale, questions related to each subdimension, F8, Data: IAC, CM, 4F, Dagstuhl; participants: experts and crowd (open crowd vs. channel partner)\\
Pilot 8: reduced dimensions, 5-point scale, questions related to each subdimension, F8, Data: CM, CMV; participants: experts and crowd (open crowd vs. channel partner)\\
Pilot 9: reduced dimensions, 5-point scale, questions related to each subdimension, F8, Data: CM, CMV; participants: crowd (channel partner only)\\
Pilot 10: reduced dimensions, 5-point scale, questions related to each subdimension, F8, Data: CM, CMV; participants: experts and crowd (channel partner only)\\
Pilot 11: yes/no for each subdimension (presented as questions), 5-point scale, F8, Data: CM + CMV, participants: experts, crowd (channel partner)\\ 
Pilot 12: score each subdimension on 3-point scale (presented as questions), 5-point scale, F8, Data: CM + CMV, participants: experts\\
- RESULTS: questions for subdimensions presented but not answered, excluding 4F (?)
\todo[color=green]{did Pilot 7 results lead to excluding 4F and using only CM and CMV for Debates?}
\paragraph{Round 4 (pilots 13-14)}
- GOAL: testing out the final annotation guidelines on the real data. "we ran one pilot on each of the new domains to identify any domain-specific issues, etc."\\
- SETUP: Pilot 13: reduced dimensions, 5-point scale, questions related to each subdimension, F8, Data: Yahoo; participants: experts\\
Pilot 14: reduced dimensions, 5-point scale, questions related to each subdimension, F8, Data: Yelp; participants: experts\\
- RESULTS: agreement table\\\\
Based on pilot results, we decided to proceed with annotation of Debate Forums, Yahoo, and Yelp data using the reduced dimensions for scoring argument quality: Cogency, Effectiveness, Reasonableness, and Overall quality.
We include questions corresponding to the subdimensions in Wachsmuth et al. [citation].
These questions were posed to annotators for their consideration when scoring each dimension, but were not scored themselves.
We use a 5-point Likert scale for scoring each dimension.

